Dynamic locational marginal emissions via implicit differentiation

Locational marginal emissions rates (LMEs) estimate the rate of change in emissions due to a small change in demand in a transmission network, and are an important metric for assessing the impact of various energy policies or interventions. In this work, we develop a new method for computing the LMEs of an electricity system via implicit differentiation. The method is model agnostic; it can compute LMEs for any convex optimization-based dispatch model, including some of the complex dispatch models employed by system operators in real electricity systems. In particular, this method lets us derive LMEs for dynamic dispatch models, i.e., models with temporal constraints such as ramping and storage. Using real data from the U.S. electricity system, we validate the proposed method against a state-of-the-art merit-order-based method and show that incorporating dynamic constraints improves model accuracy by 8.2%. Finally, we use simulations on a realistic 240-bus model of WECC to demonstrate the flexibility of the tool and the importance of incorporating dynamic constraints. Namely, static LMEs and dynamic LMEs exhibit a normalized average RMS deviation of 28.40%, implying dynamic constraints are essential to accurately modeling emissions rates.

==> bios.tex <==

\begin{IEEEbiographynophoto}{Lucas Fuentes Valenzuela}
is a Ph.D. student in the Department of Electrical Engineering at Stanford University. He received a B.S. in Engineering and an M.Sc. in Engineering Physics jointly between the University of Liege, Belgium, and CentraleSupelec, France, in 2017. 
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Anthony Degleris}
is a Ph.D. student in the Department of Electrical Engineering at Stanford University, where he is both a Stanford Graduate Fellow and a DOE Computational Science Graduate Fellow. 
His research interests is centered around optimization, long-term electricity system planning, and electricity market design.
He received a B.S. with honors in Electrical Engineering from Stanford University in 2020.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Abbas El Gamal}
(Life Fellow, IEEE)
is the Hitachi America Professor in the School of Engineering and Senior Fellow at the Precourt Institute for Energy at Stanford University. He received his M.S. in Statistics and Ph.D. in Electrical Engineering both from Stanford University in 1977 and 1978, respectively. From 1978 to 1980, he was an Assistant Professor of Electrical Engineering at USC. He has been on the faculty of the Department of Electrical Engineering at Stanford University since 1981. From 2003 to 2012, he was Director of the Information Systems Laboratory at Stanford University. From 2012-2017 he was Chair of the Department of Electrical Engineering at Stanford University. His research contributions have been in network information theory, FPGAs, digital imaging devices and systems, and smart grid modeling and control. He has authored or coauthored over 230 papers and holds 35 patents in these areas. He is coauthor of the book Network Information Theory (Cambridge Press 2011). He is a member of the US National Academy of Engineering and a Life Fellow of the IEEE. He received several honors and awards for his research contributions, including the 2016 IEEE Richard Hamming Medal and the 2012 Claude E. Shannon Award. He served on the Board of Governors of the Information Theory Society from 2009 to 2016 and was President in 2014. He cofounded and served on the board of directors and technical advisory boards of several Silicon Vally semiconductor, EDA, and biotech companies.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Marco Pavone}
(Member, IEEE) received the Ph.D. degree in aeronautics and astronautics from the Massachusetts Institute of Technology, Cambridge, MA, USA, in 2010. He is an Associate Professor of Aeronautics and Astronautics with Stanford University, Stanford, CA, USA, and the Director of Autonomous Vehicle Research with NVIDIA, Santa Clara, CA, USA. His research interests include the development of methodologies for the analysis, design, and control of autonomous systems, with an emphasis on self-driving cars, autonomous aerospace vehicles, and future mobility systems.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Ram Rajagopal}
(Member, IEEE)
is an associate professor of Civil and Environmental Engineering at Stanford University. He is the founder and director of the Stanford Sustainable Systems Lab. Ram’s primary research focus is on advancing the design, optimization and data-driven modelling of electric power systems. His work involves creating novel-sensing and control platforms, robust data processing algorithms, and dynamic statistical decision methods. He has also worked extensively on sensing infrastructure systems and transportation networks.
Ram received his Ph.D in Electrical Engineering and Computer Sciences and M.A. in Statistics from the University of California, Berkeley. He has specialized in creating and deploying large sensing systems and using the generated data together with novel statistical algorithms and stochastic control to achieve sustainable transportation, energy, and infrastructure networks.
\end{IEEEbiographynophoto}

==> body/Framework.tex <==







\newpage

\section{OLD SECTION}\label{sec:framework}

%In this section, we present a framework for computing marginal emission factors.
%First, we provide background information on convex optimization-based dispatch models in Section~\ref{sec:model}.
%We then describe our mathematical model for emissions and marginal emissions in static networks in Section~\ref{sec:mefs}. 
%Finally, in Section~\ref{sec:dyn_model}, we incorporate generic time-dependent constraints into the framework. 



% \subsection{Dispatch Model} \label{sec:model}

% In electricity systems, a \textit{dispatch model} is a mathematical model for deciding which electricity generators should be used to meet demand.
% Dispatch models can often be formulated as convex optimization problems, where the variables are the amount of generation produced by each generator, and the parameters are the electricity demand and the physical constraints of the system.
% We provide two examples below.


% We also denote by the \textit{solution map} of a parameterized optimization problem a function $g^*(\theta) : \reals^p \rightarrow \reals^k$ that maps the \textit{parameters} $\theta \in \reals^p$ of a problem to the optimal variables $g^*(\theta)$.
% In this setting, we consider problem \eqref{eq:opf} to be parameterized by $\theta = d$, and we let $g^*(d)$ be the optimal generator power outputs as a function of the demand $d$.
% Formulating the optimal solution of \eqref{eq:opf} as a function of demand enables probing the relationship between demand in generation.
% For example, the derivative $\partial_j g_i^*(d)$ quantifies how the power output at generator $i$ varies given a change in demand at node $j$ (if the derivative exists at all).
% 



%\subsection{Marginal emission factors}
%\label{sec:mefs}

%\textit{\textbf{Figure placeholder:} Figure 1. 
%A schematic diagram describing our methodology.
% (First set of frames.) First, we solve an optimization problem to dispatch the generators.
% Then, we compute the derivative via the chain rule to estimate marginal emission factors.
% (Separate frame.) Alternatively, we accumulate historical dispatch data, compute differences in generation / emissions over time, then use regression to estimate the derivative.
%}



% In this section, we introduce our model for carbon emissions.

% \paragraph{Emissions model.}
% We model the emissions of each generator as a linear function of power output, i.e., $C(g) = c^T g$.
% Although we use a linear model throughout the remainder of the paper, it is straightforward to generalize all our results to nonlinear models.
% Since the generator power outputs are determined by the dispatch model, the \textit{total emissions} generated as a function of demand is $E(d) = C(g^*(d)) = c^T g^*(d)$.

% The \textit{average emissions factor} is $\mu(d) = E(d) / (\ones^T d)$ and represents the average emissions produced per unit of power generated.
% Although average emissions factors can be helpful in quantifying the average carbon cost of energy, they do not represent how a change in electricity consumption affects carbon emissions.
% Instead, this is given by the \textit{marginal emissions factors (MEFs)}, $\lambda(d) = \nabla E(d)$, which quantifies the marginal change in carbon emissions given a marginal change in electricity demand.
% Note that $\lambda(d) \in \reals^n$ is a vector-valued function, since electricity consumption at different nodes may affect emissions differently. 

% \asdnote{Lucas: I would say that one can use this method in unknown settings -- on synthetic data. But it requires a model. This is the main point, right?}
% We then explain limitations of this method.
% Namely, (1) the data requirements and (2) the difficulty in accounting for imports and exports.


% \paragraph{Analytical formulas.}
% In simple cases, we can manually derive a simple expression for  $\partial g^*(d)$.
% For example, suppose the generator cost functions are linear functions $f_i(x) = b_i x$ in the economic dispatch model given by \eqref{eq:econ-dispatch}, and furthermore suppose no two entries of $b$ are the same, i.e., $b_i \neq b_j$ if $i \neq j$.
% Then let $\pi_1, \ldots, \pi_k$ be the permutation such that $b_{\pi_1} < b_{\pi_2} < \ldots < b_{\pi_k}$, and define $G(i) = \sum_{j=1}^i g^{\max}_i$.
% In the interval $(0, G(k))$, one can show that $\partial g^*(d)$ is defined almost everywhere\footnote{Specifically, at every point in the union of intervals $(G(0), G(1)) \cup \ldots \cup (G(k-1), G(k))$. Note that this excludes the points $G(0), \ldots, G(k)$.}, and given by 
% $$
% \partial g^*(d) 
% = \sum_{i=1}^k e_i\ \mathcal{I} \left\{ G(i-1) < d < G(i) \right\}
% $$
% where $\mathcal I$ is the indicator function.
% Although it is not made explicit, this derivation underlies the approach taken in \cite{?}.
% In other settings, an analytical expression for $\lambda(d)$ has been derived by carefully analyzing the KKT conditions of the dispatch problem~\cite{Ruiz2010AnalysisNetworks,Conejo2005LocationalSensitivities}.


 


\subsection{Dynamic dispatch models}\label{sec:dyn_model}

% Real world electricity systems often have \textit{intertemporal}, constraints that couple generator output between different time periods.
% These constraints may affect marginal emissions factors.
% For example, consider a model with \textit{ramping constraints}, which constrain the change in generation between successive time periods for certain generators.
% By drawing additional electricity and forcing a coal generator to increase its output, one may cause emissions later in the day because the generator takes additional time to ramp down.

% In this section, we describe several examples of \textit{dynamic dispatch models}, models that describe electricity system dispatch across several time periods and incorporate intertemporal constraints.
% Since our framework for computing marginal emissions factors extends to any convex optimization-based dispatch model, we can compute MEFs for dynamic dispatch models.
% As far we are aware of, this is the first work demonstrating how to compute MEFs for dynamic models.
% 
% \paragraph{Dynamic optimal power flow.}
% The \textit{dynamic optimal power flow problem} with time horizon $T$ is given by,
% \begin{equation}
% \label{eq:dyn-opf}
% \begin{array}{ll}
%     \textrm{minimize} 
%     & \sum_{t=1}^T \sum_{i=1}^k f_i((g_t)_i) \\[0.5em]
%     \textrm{subject to} 
%     & \ones^T d_t = \ones^T g_t, \quad t = 1, \ldots, T, \\
%     & 0 \leq g_t \leq g^{\max}, \quad t = 1, \ldots, T, \\
%     & \left| F (d_t - B g_t) \right| \leq p^{\max}, \quad t = 1, \ldots, T, \\
%     & \textit{(dynamic constraints)},
% \end{array}
% \end{equation}
% where the variables $g_1, \ldots, g_T \in \reals^k$ are the power produced by each generator during each time period.
% Now each time period has a unique demand $d_t \in \reals^n$ and corresponding generator output $g_t \in \reals^k$.
% Additionally, the dynamic problem has dynamic constraints that couple each time period (we denote these via \textit{(dynamic constraints)} in the problem above). 
% Without these constraints, the dynamic problem would simplify to $T$ optimal power flow problems that can be solved independently.
% Below, we describe several types of dynamic constraints that are commonly used in practice.
% 
% \paragraph{Ramping constraints.}
% Ramping constraints limit the rate at which a generator can change its output.
% These are modeled with the constraints,
% \begin{align} \label{eq:ramp-constr}
%     g_t - \rho \leq g_{t+1} \leq g_t + \rho, \quad t = 1, \ldots, T-1,
% \end{align}
% where $\rho \in \reals^k$ is the ramping rate of each generator.
% Note that we assume ramping constraints are two-sided, i.e., the down ramping rate is the same as the up ramping rate, for clarity.
% Ramping constraints are particularly useful in dynamic dispatch models with short time intervals, e.g., 15 minutes.
% 
% \paragraph{Storage constraints.}
% In dispatch models with electricity storage, we introduce new variables for the state of charge $s_t \in \reals^n$, the charge rate $r^c_t \in \reals_n$, and the discharge rate $r^d_t \in \reals^n$ at each time periods $t = 1, \ldots, T$.
% We then introduce the constraints,
% \begin{align*}
%     s_t &= s_{t-1} + \eta_c r^c_t - (1/\eta_d) r^d_t, \quad t = 1, \ldots T, \\
%     |s_t| &\leq C, \quad t = 1, \ldots T,\\
%     |r^c_t| &\leq P, \quad t = 1, \ldots T, \\
%     |r^d_t| & \leq P, \quad t = 1, \ldots T, 
% \end{align*}
% where $s_0 = 0$.
% The vector $C \in \reals^n$ is the storage capacity, $P \in \reals^n$ is the maximum (dis)charge rate, and $\eta_c, \eta_d \in (0, 1]$ are the charge and discharge efficiencies.
% In addition to adding intertemporal constraints, we also must modify the energy balance constraints $\ones^T d_t = \ones^T g_t$ and the power flow constraints $\left| F (d_t - B g_t) \right| \leq p^{\max}$ to include the charge and discharge variables,
% \begin{align*}
%     \ones^T(d_t + r^c_t) &= \ones^T(g_t + r^d_t), \\
%     \left| F (d_t + r^c_t - r^d_t - B g_t) \right| &\leq p^{\max},
% \end{align*}
% for all $t = 1, \ldots, T$.
% Adding electricity storage to a dynamic dispatch model will be particularly useful as network storage capacity increases in response to growing renewable penetration.
% 
% \paragraph{Unit commitment constraints.}
% Unit commitment constraints are integer constraints specifying whether or not a power generator is on.
% If generator $i$ is on, it must produce a minimum power $g^{\min}_i$ and stay on for a specified period of time.
% We model this by introducing an integer variable $z \in \{0, 1\}^k$ and modifying the generation constraint $0 \leq g_t \leq g^{\max}$ to include the integer constraints,
% \begin{align}
% \label{eq:unit}
%     z \odot g^{\min} \leq g_t \leq z \odot g^{\max},
% \end{align}
% where $\odot$ is elementwise multiplication.
% The integer constraint $z \in \{0, 1\}$ is nonconvex, making \eqref{eq:dyn_opf} a mixed-integer convex program.
% Fortunately, many good heuristics for mixed-integer convex programs are available through commercial solvers, such as Gurobi~\cite{?}. 
% Note that differentiating the solution map $g^*(d)$ requires slight modifications in the mixed-integer case; see Appendix~\ref{?}. 


\begin{comment}
\section{Old}
In this section, we describe our model for the energy market and emissions.
Our model for the energy market---namely, a DC optimal power flow model \cite{?LecNote}---is commonly used in the literature and in practice.
Moreover, our results are all easy to extend to more detailed models, e.g.\ an AC optimal power flow model.
Finally, we conclude the section by briefly explaining how to compute the sensitivities of emissions with respect to network parameters and inputs.
This is accomplished by differentiating the solution mapping via the implicit function theorem.

\paragraph{Energy market.}
We consider a simple DC optimal power flow model for the energy market.
Consider a network with $n$ nodes, $m$ edges, and $\ell$ generators, described by the incidence matrix $A \in \reals^{n \times m}$ and a node-generator map $B \in \reals^{n \times \ell}$.
The variables of the optimization problem are the generations of each generator, $g \in \reals^\ell$, the power flows across each edge, $p \in \reals^m$, and the voltage phase angles $v \in \reals^n$.
The generation at generator $i$ is limited by its capacity, $0 \leq g_i \leq g^{\max}_i$, and has cost $c^q_i g_i^2 + c^\ell_i g_i$.
Each power flow $p_j$ has a capacity constraint $|p_j| \leq p^{\max}_j$ and is determined by the difference of phase angles, i.e.\ $p = \diag(\gamma) A^T v$, where $\gamma_j \in \reals_+$ is the susceptance of line $j$.
Finally, each node $i$ has energy demand $d_i \in \reals$, and the network must satisfy power balance, $B g - d = Ap$.
In total, the \textit{optimal power flow} problem is,
\begin{equation} \label{eq:opf}
\begin{array}{ll}
    \text{minimize} & g^T \diag(c^q) g + g^T c^\ell \\
    \text{subject to} 
    & 0 \leq g \leq g^{\max}, \\
    & |p| \leq p^{\max}, \\
    & p = \diag(\gamma) A^T v, \\
    & B g - d = Ap,
\end{array}
\end{equation}
where the variables are $g, v \in \reals^n$ and $p \in \reals^m$.
Here, all inequalities are to be read elementwise.


\paragraph{Emissions.}
For the purpose of simplicity, we model emissions as a linear function of generation.
Specifically, each generator emits $b_i \in \reals_+$ units per unit of generation, and the total emissions are $E(g) = b^T g$.


\subsection{Computing sensitivities} \label{sec:sensitivity}

The \textit{sensitivity} of a function $f(x) : \reals^n \rightarrow \reals$ is given by its gradient $\nabla f(x)$, which tells us how $f(x)$ changes given a small change in $x$.
Computing the sensitivity of emissions $E(g)$ to generation is easy, since $\nabla E(g) = b$.
However, generation is indirectly determined by the parameters of \eqref{eq:opf}, like demand $d$, prices $f^q, f^\ell$, and capacities $p^{\max}$.
Computing the sensitivity of emissions to $d$, for example, is more difficult, since it's not immediately clear how $d$ affects $g$.

\paragraph{Solution mapping.}
Let $\theta = (d, f^q, f^\ell, g^{\max}, p^{\max}, \gamma) \in \reals^{k}$ be the \textit{parameters} or \textit{inputs} of \eqref{eq:opf}.
Then let $g^*(\theta) : \reals^k \rightarrow \reals^n$ be the \textit{solution mapping} that maps $\theta$ to the optimal value of $g$ in \eqref{eq:opf} when the problem data is set to $\theta$.
Finally, define $\tilde E(\theta) = E(g^*(\theta))$ to be emissions as a function of the parameters $\theta$.
Assuming $g^*$ is well-defined and differentiable, computing $\nabla \tilde E(\theta)$ gives us a rigorous approach to finding the sensitivity of emissions to various problem parameters.
It is often useful to let $\theta$ be a subset of the problem data, e.g.\ $\theta = d$, and consider all other problem data fixed.
We will therefore sometimes abuse notation and write $g^*(d)$ or $g^*(p^{\max})$, for example, to signal to the reader that $\theta = d$ or $\theta = p^{\max}$, respectively, and all other problem data are fixed.

\paragraph{Implicit differentiation.}
The chain rule tells us that $\nabla \tilde E(\theta) = \partial g^*(\theta)^T b$.
The main technical challenge is computing the Jacobian $\partial g^*(\theta)$, if it even exists.
It turns out that we can do this assuming $g^*$ is well-defined (i.e.\ the solution to \eqref{eq:opf} is unique) in some local neighborhood around $\theta$.
In particular, we view the solution of \eqref{eq:opf} as the solution to a system of equations $K(x, \theta) = 0$ (namely, the KKT conditions), then invoke the \textit{implicit function theorem} to compute the Jacobian matrix $\partial g^*(\theta) \in \reals^{n \times k}$.
Computing said Jacobian is also relatively efficient---after solving \eqref{eq:opf}, which is already required to compute $g^*(\theta)$, the Jacobian is easy and fast to evaluate.
For completeness, we include additional details in the appendix.






\section{Marginal emission factors} \label{sec:mefs}

In this section, we describe an important metric in emissions analysis---marginal emission factors (MEFs).
We first review the standard method for computing MEFs, then show how our sensitivity-based approach recovers the same quantity.
Finally, we explain how our approach allows one to compute \textit{dynamic} marginal emission factors, i.e.\ MEFs that incorporate temporal information.
As far as we know, dynamic MEFs have yet to be established in the literature, likely because computing dynamic MEFs is statistically or computationally intractable using traditional.

\paragraph{Static marginal emission factors.}
The \textit{marginal emission factor} at node $i$ is the marginal change in emissions given a marginal change in demand at node $i$.
Mathematically, given demand vector $d$, the marginal emission factor $\mu_i(d)$ at node $i$ is such that $E(g^*(d + \delta) ) \approx E(g^*(d)) + \mu(d)^T\delta$, i.e.\ the (locally) linear change in emissions given a change in demand.

\paragraph{Traditional methods.}
Traditionally, two approaches have been used to compute MEFs \cite{?}.
The first approach is regression-based.
In particular, after observing demand vectors $d^{(1)}, \ldots, d^{(T)}$ and corresponding emissions $E^{(1)}, \ldots, E^{(T)}$, we solve $n$ linear regression problems $\mu_i(d) =  \mathrm{argmin}_{\alpha}\ \frac{1}{2} \sum_{t=1}^T (E^{(t)} - \alpha d_i^{(t)})^2$ to recover $\mu(d)$.
This approach works well when an abundance of data is available and the demands at each node are mostly uncorrelated. \anthony{I'll need to revise this a bit. Talk more about the limitations / data requirements. Mention how this ignores imports / exports.}

The second approach is simulation-based.
To determine the MEF $\mu_i(d)$, we compute $E(g^*(d))$ and $E(g^*(d + \epsilon e_i))$, where $\epsilon > 0$ is small.
Then $\mu_i(d) \approx \left(E(g^*(d + \epsilon e_i)) - E(g^*(d)) \right) / \epsilon$.
The main limitation of this method is that it requires solving \eqref{eq:opf} $n+1$ times to compute the MEF at each node; for large networks, this quickly becomes intractable, especially when the MEFs need to be computed for various operating conditions (e.g.\ different seasons, different times of day).
\anthony{TODO Fact check!}

\paragraph{Sensitivity method.}
As the reader may have noticed, the definition of the MEFs $\mu(d)$ are exactly the gradient $\nabla \tilde E(d)$.
Therefore, we propose leveraging the techniques presented in Section~\ref{sec:sensitivity} to directly compute $\mu(d) = \nabla \tilde E(d)$.
This method is still simulation-based, but only requires solving \eqref{eq:opf} once, instead of $n+1$ times, making it computationally tractable even for very large networks.
Moreover, our approach precisely captures the mathematical definition of MEFs---in fact, if $\tilde E(d)$ is not locally differentiable near $d$, the MEF $\mu(d)$ does not make sense, since the marginal change in emissions is not unique.

\paragraph{Modeling more complex markets.}
Real electricity markets often include additional constraints, such as reliability constraints (e.g.\ the $N-1$ security constraint) and unit commitment constraints.
Consequently, mathematically derived MEFs specific to a particular energy market model are limited in practice.
Our method, in contrast, applies to any optimization-based model for the energy market.
Because we use automatic differentiation to compute derivatives and Jacobians, the only change required to modify our framework for different dispatch models is to change the definition of \eqref{eq:opf}, and update the KKT operator $K(x, \theta)$ accordingly.
In the following section, we will show how this flexibility lets us model \textit{dynamic} energy markets, that is, markets with energy storage that are coupled in time.
This let's us compute a variant of marginal emission factors that account for \textit{delayed emissions}, emissions produced earlier or later in time because of a change in demand now.




\section{Dynamic marginal emission factors.} \label{sec:dyn-mef}



\paragraph{Dynamic energy market.} We introduce an extension of the model in~\eqref{eq:opf} that introduces storage into the system. The presence of storage introduces dependencies between subsequent timesteps. We also see the introduction of additional nodal variables $s_t$ indicating the state of charge of \say{nodal storage} at timestep $t$. They are constrained by a maximum charge of $C$ and a maximum charge/discharge power $P$. 
% \lucas{For the moment, I neglect the equation with $v_t$ for the sake of simplicity}

\begin{equation} \label{eq:dyn_opf}
\begin{array}{ll}
    \text{minimize} & \sum_t (g_t^T \diag(c^q) g_t + g_t^T c^\ell) \\
    \text{subject to} 
    & 0 \leq g_t \leq g_t^{\max}, \\
    & |p_t| \leq p_t^{\max}, \\
    & p_t = \diag(\gamma) A^T v_t \\
    % & p_t = \diag(\gamma) A^T v_t, \\
    & B g_t - d_t - (s_t - s_{t-1}) = Ap_t,\\
    & 0 \leq s_t \leq C, \\
    & | s_t - s_{t-1}| \leq P, \ t = 1, ...T\\
    & s_0 = C_0
\end{array}
\end{equation}




\end{comment}





% \section{Carbon-aware planning} \label{sec:planning}
